Reconfigurable and approximate computing for video coding

The Chapter begins with a discussion of the constraints and needs of video coding systems. The lack in flexibility of traditional monolithic codec specifications, not suitable to model commonalities among codecs and foster reusability among successive codec generations/updates, was the main trigger for the development of a new standard initiative within the ISO/IEC MPEG committee, called reconfigurable video coding (RVC). The MPEG-RVC framework exploits the dataflow nature behind video coding to foster flexible and reconfigurable codec design, as well as to support dynamic reconfiguration. The Chapter goes on to consider that the inherent resiliency of various functional blocks (like motion estimation in the high-efficiency video coding, HEVC) and the varying levels of user perception make video coding suitable to apply approximate computing techniques. Approximate computing, if properly supported at design time, allows achieving run-time trade-offs, representing a new direction in hardware-software codesign research. The main assumption behind approximate computing, exploited within video coding, is that the degree of accuracy (in this case during codec execution) is not required to be the same all the time. The final part of the Chapter attempts to put together the concepts addressed and remarks on which are, in the authors' opinion, some interesting research directions.

==> IET - Book Chapter/acronyms.tex <==
% A
\newacronym{asm}{ASM}{Assembly}

% B
\newacronym{bpdf}{BPDF}{Boolean Parametric Dataflow}

% C
\newacronym{cal}{CAL}{CAL Actor Language}
\newacronym{cfdf}{CFDF}{Core-Functional Dataflow}
\newacronym{csdf}{CSDF}{Cyclo-Static Dataflow}
\newacronym{cpu}{CPU}{Central Processing Unit}

% D
\newacronym{dpn}{DPN}{Dataflow Process Network}

% F
\newacronym{fifo}{F\textsc{ifo}}{First-In First-Out queue}
\newacronym{fsm}{FSM}{Finite State Machine}

% G
\newacronym{gpu}{GPU}{Graphics Processing Unit}
\newacronym{gcd}{GCD}{Greatest Common Divisor}

% I
\newacronym{ir}{IR}{Intermediate Representation}

% J
\newacronym{jade}{\textsc{Jade}}{Just-in-time Adaptive Decoder Engine}

% L
\newacronym{lte}{LTE}{Long-Term Evolution}

% M
\newacronym[longplural=Models of Computation]{moc}{MoC}{Model of Computation}
\newacronym[longplural=Multiprocessor Systems-on-Chips]{mpsoc}{MPSoC}{Multiprocessor System-on-Chip}
\newacronym{mdsdf}{MDSDF}{Multi-Dimensional \gls{sdf}}
\newacronym{mpeg}{MPEG}{Motion Picture Expert Group}

% O
\newacronym{ofdm}{OFDM}{Orthogonal Frequency-Division Multiplexing}

% P
\newacronym{pagpan}{P-AGPAN}{Parameterized Acyclic Pairwise Grouping of Adjacent Nodes}
\newacronym{padaf}{\textsc{p}a\textsc{d}a\textsc{f}}{Parametric Dataflow Format}
\newacronym{pe}{PE}{Processing Element}
\newacronym{pimm}{PiMM}{Parameterized and Interfaced Dataflow Meta-Model}
\newacronym{pisdf}{{\Large$\pi$}SDF}{Parameterized and Interfaced \gls{sdf}}
\newacronym{preesm}{\textsc{Preesm}}{Parallel Real-time Embedded Executives Scheduling Method}
\newacronym{psdf}{PSDF}{Parameterized \gls{sdf}}
\newacronym{psm}{PSM}{Parameterized Set of Modes}

% R
\newacronym{rtos}{RTOS}{Real-Time Operating System}

% S
\newacronym{sadf}{SADF}{Scenario-Aware Dataflow}
\newacronym{sdf}{SDF}{Synchronous Dataflow}
\newacronym{sdr}{SDR}{Software Defined Radio}
\newacronym{spdf}{SPDF}{Schedulable Parametric Dataflow}
\newacronym{spider}{\textsc{Spider}}{Synchronous Parameterized and Interfaced Dataflow Embedded Runtime}

